Orthogonal AMP

Approximate message passing (AMP) is a low-cost iterative signal recovery algorithm for linear system models. When the system transform matrix has independent identically distributed (IID) Gaussian entries, the performance of AMP can be asymptotically characterized by a simple scalar recursion called state evolution (SE). However, SE may become unreliable for other matrix ensembles, especially for ill-conditioned ones. This imposes limits on the applications of AMP. In this paper, we propose an orthogonal AMP (OAMP) algorithm based on de-correlated linear estimation (LE) and divergence-free non-linear estimation (NLE). The Onsager term in standard AMP vanishes as a result of the divergence-free constraint on NLE. We develop an SE procedure for OAMP and show numerically that the SE for OAMP is accurate for general unitarily-invariant matrices, including IID Gaussian matrices and partial orthogonal matrices. We further derive optimized options for OAMP and show that the corresponding SE fixed point coincides with the optimal performance obtained via the replica method. Our numerical results demonstrate that OAMP can be advantageous over AMP, especially for ill-conditioned matrices

==> SE.tex <==
\section{State Evolution for OAMP}\label{Sec:IV}
In this section, we analyze the performance of OAMP using state evolution.
\subsection{State Evolution for OAMP}
Define
\BS \label{Eqn:IV-A-SE}
\begin{align}
\Phi_t\left( {v_t^2 } \right) &\equiv \frac{{{\rm{E}}\left\{ {g_t^2  \cdot \lambda ^2 } \right\} \cdot v_t^2  + {\rm{E}}\left\{ {g_t^2  \cdot \lambda } \right\} \cdot \sigma ^2 }}{{\left[ {{\rm{E}}\left\{ {g_t  \cdot \lambda } \right\}} \right]^2 }} - v_t^2 , \label{Eqn:IV-A-SE-a} \\
\Psi _t \left( {\tau _t^2 } \right) &\equiv {\rm{E}}\left\{ {\left( {\eta _t \left( {X + \tau _t Z} \right) - X} \right)^2 } \right\}, \label{Eqn:IV-A-SE-b}\\
\Psi _t^{{\rm{out}}} \left( {\tau _t^2 } \right) &\equiv {\rm{E}}\left\{ {\left( {\eta _t^{{\rm{out}}} \left( {X + \tau _t Z} \right) - X} \right)^2 } \right\},\label{Eqn:IV-A-SE-c}
\end{align}
\ES
where $g_t$ represents $g_t(\lambda,v_t^2)$ and $\eta_t(r)=C_t\big[\hat{\eta}_t(r)-\mr{E}\{\hat{\eta}'_t(X+\tau_tZ)\cdot r\}\big]$ (see \eqref{Eqn:III-A-DF-fun} and \eqref{Eqn:III-B-OAMP-DF}). The expectation in \eqref{Eqn:IV-A-SE} is taken over $\lambda$ w.r.t. the asymptotic eigenvalue distribution of $\bm{A}^{\mr{T}}\bm{A}$ (\textit{including the zero eigenvalues}) and the expectations in \eqref{Eqn:IV-A-SE-b} and \eqref{Eqn:IV-A-SE-c} are taken over $X\sim P_X(x)$ and $Z\sim \mathcal{N}(0,1)$. \par
Starting with $v_0^2=\mr{E}\{X^2\}$, the SE for OAMP is given by the following recursion
\BS \label{Eqn:IV-A-SE2}
\begin{align}
\tau _t^2  &= \Phi _t \left( {v_t^2 } \right),\\
v_{t + 1}^2 & = \Psi _t \left( {\tau _t^2 } \right).
\end{align}
\ES
\par
Under the condition that $\bm{A}$ is unitarily invariant and $\bm{W}_t$ is given by \eqref{Eqn:III-C-linear2}, we conjecture that the following holds for OAMP (similar to Theorem 1). \vspace{5pt}
\begin{conjecture}
The OAMP algorithm in \eqref{Eqn:III-B-OAMP} can be characterized by the SE in \eqref{Eqn:IV-A-SE2}.
\end{conjecture}\vspace{5pt}\par
Currently, we still cannot complete a rigorous proof for Conjecture 1. Nevertheless, we will provide numerical evidence for Conjecture 1 in Section~\ref{Sec:VI}. \par Notice that the estimate for $\bm{x}$ of OAMP is generated by $\eta_t^{\mr{out}}$ rather than $\eta_t$. From Conjecture 1, the MSE performance of OAMP is given by
\BE \label{Eqn:IV-A-out}
\frac{1}{N}\left\| {\eta _t^{{\rm{out}}} \left( {{\bf{r}}^t } \right) - {\bf{x}}} \right\|^2  \to \Psi _t^{{\rm{out}}} \left( {\tau _t^2 } \right),
\EE
where $\Psi _t^{{\rm{out}}}$ is defined in \eqref{Eqn:IV-A-SE-c}.
%======================================================================================
\subsection{Heuristic Derivations of SE} \label{Sec:IV-B}
Similar to \eqref{Eqn:II-B-1}, define
\BE \label{Eqn:IV-B-1}
\bm{q}^t\equiv\bm{x}^t-\bm{x}\text{ and } \bm{h}^t\equiv\bm{r}^t-\bm{x}.
\EE
Based on \eqref{Eqn:IV-B-1}, we can rewrite \eqref{Eqn:III-B-OAMP} as\par
\textit{OAMP Error Recursion:}
\BS \label{Eqn:IV-B-error}
\begin{align}
{\bf{h}}^t & = \left( {{\bf{I}} - \alpha _t {\bf{W}}_t {\bf{A}}} \right){\bf{q}}^t  + \alpha _t {\bf{W}}_t {\bf{n}}, \label{Eqn:IV-B-error-a}\\
{\bf{q}}^{t + 1}  &= \eta _t \left( {{\bf{x}} + {\bf{h}}^t } \right) - {\bf{x}}.\label{Eqn:IV-B-error-b}
\end{align}
\ES
The SE in \eqref{Eqn:IV-A-SE2} tracks the behavior of $v_t^2$ and $\tau_t^2$, which can be intuitively interpreted as
 \BE \label{Eqn:IV-B-variances}
v_t^2  = \frac{1}{N}\cdot{\rm{E}}\left\{ {\left\| {{\bf{q}}^t } \right\|^2 } \right\}{\text{ and }}\tau _t^2  = \frac{1}{N}\cdot{\rm{E}}\left\{ {\left\| {{\bf{h}}^t } \right\|^2 } \right\}.
 \EE\par
The SE equations in \eqref{Eqn:IV-A-SE2} are derived based on Assumptions 1-2 below. The details can be found in Appendix~\ref{App:I}. Note that Assumptions 1-2 generally do not hold exactly. However, they provide useful intuitions to understand the SE recursions.

\begin{assumption}
In \eqref{Eqn:IV-B-error}, $\bm{q}^t$ consists of IID entries with $\mr{E}\big\{(q_j^t)^2\big\}=v_t^2$, and $\bm{q}^t$ is independent of $\bm{A}$ and $\bm{n}$.
\end{assumption}\par \vspace{5pt}

\begin{assumption}
In \eqref{Eqn:IV-B-error}, $\bm{h}^t$ consists of IID entries with $h_j^t\sim\mathcal{N}(0,\tau_t^2)$, and $\bm{h}^t$ is independent of $\bm{x}$.
\end{assumption}\par \vspace{5pt}

Our intuition to design the OAMP algorithm in \eqref{Eqn:III-B-OAMP} is based on two considerations. First, the introduction of $\alpha_t$ in \eqref{Eqn:III-B-OAMP-a} de-correlates $\bm{x}$ and $\bm{h}^t$, which partially justifies Assumption 2 (Assumption 2 is stronger).


\begin{proposition}\label{Pro:IV}
Under Assumption 1, $\bm{x}$ and $\bm{h}^t$ are uncorrelated when $\bm{A}$ is unitarily-invariant.
\end{proposition}
\begin{proof}
See Appendix~\ref{App:II}.
\end{proof}
\par
Second, the DF requirement on $\eta_t$ ``de-correlates" $\bm{q}^{t+1}$ and $\bm{A}$, which further provides a useful clue for Assumption 1 for the $t+1$-th iteration. Note that the statistical dependency on $\bm{A}$ is inherited from $\bm{h}^t$ to $\bm{q}^{t+1}$ (through the function $\eta_t(\bm{x}+\bm{h}^t) - \bm{x}$). We need to ``break" this passing of correlations to ensure Assumption 1 in the next iteration. Note that if $\bm{q}^{t+1}$ is independent of $\bm{h}^t$, then it is also independent of $\bm{A}$ from the Markovian property $\bm{A}\to\bm{h}^t\to\bm{q}^{t+1}$. However, $\bm{q}^{t+1}$ and $\bm{h}^t$ cannot be independent as $\bm{q}^{t+1}$ is a deterministic function of $\bm{h}^t$. Nevertheless, we can make $\bm{q}^{t+1}$ and $\bm{h}^t$ uncorrelated by requiring $\eta_t$ to be DF. This follows from Assumption 2 and \eqref{Eqn:III-A-orth3}.

%=========================================================================================================
\subsection{MSE Estimation}\label{Sec:IV-C}
In OAMP, $v_t^2$ and $\tau_t^2$ are in general parameters of $\bm{W}_t$, $\eta_t$ and $\eta_t^{\mr{out}}$, (see \eqref{Eqn:V-A-opt} in Section~\ref{Sec:V}). If the statistical distributions of $\lambda(\bm{A}^{\mr{T}}\bm{A})$ and $\bm{x}$ are known, then $v_t^2$ and $\tau_t^2$ can be computed from the SE equations in \eqref{Eqn:IV-A-SE}. On the other hand, if the distributions of $\lambda(\bm{A}^{\mr{T}}\bm{A})$ and $\bm{x}$ are unknown, $v_t^2$ and $\tau_t^2$ can still be estimated as follows.\par
For $v_t^2$, we adopt the following estimator \cite[Eqn.~(71)]{Vila2013}
\BE \label{Eqn:IV-C-MSE1}
\hat v_t^2  = \frac{{\left\| {{\bf{y}} - {\bf{Ax}}^t } \right\|{}^2 - M \cdot \sigma ^2 }}{{{\rm{tr}}\left( {{\bf{A}}^{\rm{T}} {\bf{A}}} \right)}}.
\EE
Note that $\hat{v}_t^2$ in \eqref{Eqn:IV-C-MSE1} can be negative. We may use $\max(\hat{v}_t^2,\epsilon)$ as a practical estimator for $v_t^2$, where $\epsilon$ is a small positive constant. (Setting $\epsilon=0$ may cause a stability problem.)\par
Given $\hat{v}_t^2$, $\tau_t^2$ can be estimated using the empirical form of \eqref{Eqn:IV-A-SE-b}:
\BE \label{Eqn:IV-C-MSE2}
\hat \tau _t^2  = N \cdot \left( {\frac{{{\rm{tr}}\left\{ {\left( {{\bf{W}}_t {\bf{A}}} \right)^2 } \right\} \cdot \hat v_t^2  + {\rm{tr}}\left\{ {{\bf{W}}_t {\bf{W}}_t^{\rm{T}} } \right\} \cdot \sigma ^2 }}{{\left( {{\rm{tr}}\left\{ {{\bf{W}}_t {\bf{A}}} \right\}} \right)^2 }}} \right) - \hat v_t^2 .
\EE
Eqn.~\eqref{Eqn:IV-C-MSE2} can be simplified to more concise formulas for some choices of $\bm{W}_t$. For example, \eqref{Eqn:IV-C-MSE2} simplifies to $\hat \tau _t^2  = \left( {N - M} \right)/M \cdot \hat v_t^2  + N/M^2  \cdot {\rm{tr}}\big\{ {\left( {{\bf{AA}}^{\rm{T}} } \right)^{ - 1} } \big\} \cdot \sigma ^2$ when $\bm{W}_t$ is the PINV estimator given in \eqref{Eqn:III-C-linear1-b}.\par
The numerical results presented in Section~\ref{Sec:VI} are obtained based on approximations in \eqref{Eqn:IV-C-MSE1} and \eqref{Eqn:IV-C-MSE2}.

